Decision Support for the Quickest Detection of Critical COVID-19 Phases

During the course of an epidemic, one of the most challenging tasks for authorities is to decide what kind of restrictive measures to introduce and when these should be enforced. In order to take informed decisions in a fully rational manner, the onset of a critical regime, characterized by an exponential growth of the contagion, must be identified as quickly as possible. Providing rigorous quantitative tools to detect such an onset represents an important contribution from the scientific community to proactively support the political decision makers. In this paper, leveraging the quickest detection theory, we propose a mathematical model of the COVID-19 pandemic evolution and develop decision tools to rapidly detect the passage from a controlled regime to a critical one. A new sequential test -- referred to as MAST (mean-agnostic sequential test) -- is presented, and demonstrated on publicly available COVID-19 infection data from different countries. Then, the performance of MAST is investigated for the second pandemic wave, showing an effective trade-off between average decision delay $\Delta$ and risk $R$, where $R$ is inversely proportional to the time required to declare the need to take unnecessary restrictive measures. Ideally, the decision mechanism should react as quick as possible for a given level of risk. We find that all the countries share the same behaviour in terms of quickest detection, specifically the risk scales exponentially with the delay, $R \sim \exp{(-\omega \Delta)}$, where $\omega$ depends on the specific nation. For a reasonably small risk level, say, one possibility in ten thousand (i.e., unmotivated implementation of countermeasures every 27 years, on the average), the proposed algorithm detects the onset of the critical regime with delay between a few days to three weeks, much earlier than when the exponential growth becomes evident.

==> figures/France-delay-and-fa-vs-thr.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Threshold}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{8mm}{\hspace{0mm}{Delay [days]}}}
%
%
\psfrag{leg1}[l][l]	[\commonScale]{	\raisebox{0mm}{\hspace{-1mm}{Operational Curve}}}
\psfrag{leg2}[l][l]	[\commonScale]{	\raisebox{0mm}{\hspace{-1mm}{$p_{n}$ -- Moving average applied to $\tilde{p}_{n}$}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-5mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff $0$}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff $5$}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff $10$}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff $15$}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff $20$}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff $25$}}
\psfrag{x7}[c][c]	[\xscale]{	\xvoff{\xhoff $30$}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.05$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.10$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.15$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.20$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.25$}}

%
\psfrag{yr1}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $0$}}
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $10$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $20$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $30$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $40$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $50$}}
\psfrag{yr7}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $60$}}
\psfrag{yr8}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $70$}}

==> figures/France-new-positives-shade.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{10mm}{\hspace{0mm}{\# Individuals (in thousands)}}}
%
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Daily new positive cases}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{$p_{n}$ -- Smoothing of the above}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Mar}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $20$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $40$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $60$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $80$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $100$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $120$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $140$}}

==> figures/France-ratio.tex <==
\newcommand{\commonScale}{.75}
%
\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{15mm}{\hspace{0mm}{Growth Rate}}}
%
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{$x_{n}$ -- Growth rate}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Smoothing of the above}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff Mar}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0.7$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $0.8$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $0.9$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $1.0$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $1.1$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $1.2$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $1.3$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $1.4$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $1.5$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff $1.6$}}

==> figures/France-test-wave-2-non-uniform.tex <==
\newcommand{\commonScale}{1}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Stopping Day}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{12mm}{\hspace{0mm}{Delay [days]}}}
%
\newcommand{\xscale}{.85}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.85}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $\leqslant 10^{-9}$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-8}$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-7}$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-6}$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-5}$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-4}$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-3}$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-2}$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-1}$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $1$}}
%
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $10$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $20$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $30$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $40$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $50$}}
\psfrag{yr7}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $60$}}
\psfrag{yr8}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $70$}}
\psfrag{yr9}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $80$}}
\psfrag{yr10}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $90$}}
\psfrag{yr11}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $100$}}
\psfrag{yr12}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $110$}}
\psfrag{yr13}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $120$}}
\psfrag{yr14}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $130$}}
\psfrag{yr15}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $140$}}

==> figures/Germany-delay-and-fa-vs-thr.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Threshold}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{8mm}{\hspace{0mm}{Delay [days]}}}
%
%
\psfrag{leg1}[l][l]	[\commonScale]{	\raisebox{0mm}{\hspace{-1mm}{Operational Curve}}}
\psfrag{leg2}[l][l]	[\commonScale]{	\raisebox{0mm}{\hspace{-1mm}{$p_{n}$ -- Moving average applied to $\tilde{p}_{n}$}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-5mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff $0$}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff $5$}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff $10$}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff $15$}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff $20$}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff $25$}}
\psfrag{x7}[c][c]	[\xscale]{	\xvoff{\xhoff $30$}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.01$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.02$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.03$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.04$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.05$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.06$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.07$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.08$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.09$}}
%
\psfrag{yr1}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $0$}}
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $5$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $10$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $15$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $20$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $25$}}
\psfrag{yr7}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $30$}}
\psfrag{yr8}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $35$}}

==> figures/Germany-new-positives-shade.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{10mm}{\hspace{0mm}{\# Individuals (in thousands)}}}
%
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Daily new positive cases}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{$p_{n}$ -- Smoothing of the above}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Mar}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $5$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $10$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $15$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $20$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $25$}}

==> figures/Germany-ratio.tex <==
\newcommand{\commonScale}{.75}
%
\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{15mm}{\hspace{0mm}{Growth Rate}}}
%
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{$x_{n}$ -- Growth rate}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Smoothing of the above}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff Mar}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0.9$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $1.0$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $1.1$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $1.2$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $1.3$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $1.4$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $1.5$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $1.6$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $1.7$}}

==> figures/Germany-test-wave-3-non-uniform.tex <==
\newcommand{\commonScale}{1}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Stopping Day}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{12mm}{\hspace{0mm}{Delay [days]}}}
%
\newcommand{\xscale}{.85}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.85}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $\leqslant 10^{-9}$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-8}$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-7}$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-6}$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-5}$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-4}$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-3}$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-2}$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-1}$}}
%
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $10$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $20$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $30$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $40$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $50$}}
\psfrag{yr7}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $60$}}
\psfrag{yr8}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $70$}}
\psfrag{yr9}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $80$}}
\psfrag{yr10}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $90$}}
\psfrag{yr11}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $100$}}
\psfrag{yr12}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $110$}}
\psfrag{yr13}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $120$}}
\psfrag{yr14}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $130$}}
\psfrag{yr15}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $140$}}
\psfrag{yr16}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $150$}}
\psfrag{yr17}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $160$}}
\psfrag{yr18}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $170$}}
\psfrag{yr19}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $180$}}

==> figures/Italy-Hospitalized-ratio.tex <==
\newcommand{\commonScale}{.75}
%
\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{15mm}{\hspace{0mm}{Growth Rate}}}
%
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Growth rate ``hospitalized individuals''}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Smoothing of the above}}}
\psfrag{leg3}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Growth rate ``daily new positives''}}}
\psfrag{leg4}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Smoothing of the above}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff Mar}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0.8$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $1.0$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $1.2$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $1.4$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $1.6$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $1.8$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $2.0$}}

==> figures/Italy-Hospitalized-test-all-waves-non-uniform.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Stopping Day}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{12mm}{\hspace{0mm}{Delay [days]}}}
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{MAST on ``daily new positives''}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{MAST on ``hospitalized individuals''}}}
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $\leqslant 10^{-9}$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-8}$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-7}$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-6}$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-5}$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-4}$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-3}$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-2}$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-1}$}}
%
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $10$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $20$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $30$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $40$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $50$}}
\psfrag{yr7}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $60$}}
\psfrag{yr8}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $70$}}
\psfrag{yr9}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $80$}}
\psfrag{yr10}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $90$}}
\psfrag{yr11}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $100$}}
\psfrag{yr12}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $110$}}
\psfrag{yr13}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $120$}}
\psfrag{yr14}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $130$}}
\psfrag{yr15}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $140$}}
\psfrag{yr16}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $150$}}
\psfrag{yr17}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $160$}}
\psfrag{yr18}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $170$}}
\psfrag{yr19}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $180$}}
\psfrag{yr20}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $190$}}
\psfrag{yr21}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $200$}}
\psfrag{yr22}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $210$}}
\psfrag{yr23}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $220$}}
\psfrag{yr24}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $230$}}
\psfrag{yr25}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $240$}}
\psfrag{yr26}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $250$}}

==> figures/Italy-delay-and-fa-vs-thr.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Threshold}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{8mm}{\hspace{0mm}{Delay [days]}}}
%
%
\psfrag{leg1}[l][l]	[\commonScale]{	\raisebox{0mm}{\hspace{-1mm}{Operational Curve}}}
\psfrag{leg2}[l][l]	[\commonScale]{	\raisebox{0mm}{\hspace{-1mm}{$p_{n}$ -- Moving average applied to $\tilde{p}_{n}$}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-5mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff $0$}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff $5$}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff $10$}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff $15$}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff $20$}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff $25$}}
\psfrag{x7}[c][c]	[\xscale]{	\xvoff{\xhoff $30$}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.005$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.010$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.015$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.020$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.025$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.030$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.035$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.040$}}
%
\psfrag{yr1}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $0$}}
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $2$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $4$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $6$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $8$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $10$}}
\psfrag{yr7}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $12$}}
\psfrag{yr8}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $14$}}

==> figures/Italy-new-positives-shade.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{10mm}{\hspace{0mm}{\# Individuals (in thousands)}}}
%
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Daily new positive cases}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{$p_{n}$ -- Smoothing of the above}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Mar}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $5$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $10$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $15$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $20$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $25$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $30$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $35$}}

==> figures/Italy-ratio.tex <==
\newcommand{\commonScale}{.75}
%
\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{15mm}{\hspace{0mm}{Growth Rate}}}
%
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{$x_{n}$ -- Growth rate}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Smoothing of the above}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff Mar}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0.90$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $0.95$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $1.00$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $1.05$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $1.10$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $1.15$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $1.20$}}

==> figures/Italy-test-wave-2-non-uniform.tex <==
\newcommand{\commonScale}{1}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Stopping Day}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{12mm}{\hspace{0mm}{Delay [days]}}}
%
\newcommand{\xscale}{.85}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.85}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $\leqslant 10^{-9}$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-8}$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-7}$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-6}$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-5}$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-4}$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-3}$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-2}$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-1}$}}
%
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $10$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $20$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $30$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $40$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $50$}}
\psfrag{yr7}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $60$}}
\psfrag{yr8}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $70$}}
\psfrag{yr9}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $80$}}
\psfrag{yr10}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $90$}}
\psfrag{yr11}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $100$}}
\psfrag{yr12}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $110$}}
\psfrag{yr13}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $120$}}
\psfrag{yr14}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $130$}}
\psfrag{yr15}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $140$}}
\psfrag{yr16}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $150$}}
\psfrag{yr17}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $160$}}
\psfrag{yr18}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $170$}}
\psfrag{yr19}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $180$}}
\psfrag{yr20}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $190$}}
\psfrag{yr21}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $200$}}
\psfrag{yr22}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $210$}}
\psfrag{yr23}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $220$}}
\psfrag{yr24}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $230$}}
\psfrag{yr25}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $240$}}
\psfrag{yr26}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $250$}}

==> figures/US-delay-and-fa-vs-thr.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Threshold}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{8mm}{\hspace{0mm}{Delay [days]}}}
%
%
\psfrag{leg1}[l][l]	[\commonScale]{	\raisebox{0mm}{\hspace{-1mm}{Operational Curve}}}
\psfrag{leg2}[l][l]	[\commonScale]{	\raisebox{0mm}{\hspace{-1mm}{$p_{n}$ -- Moving average applied to $\tilde{p}_{n}$}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-5mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff $0$}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff $2$}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff $4$}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff $6$}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff $8$}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff $10$}}
\psfrag{x7}[c][c]	[\xscale]{	\xvoff{\xhoff $12$}}
\psfrag{x8}[c][c]	[\xscale]{	\xvoff{\xhoff $14$}}
\psfrag{x9}[c][c]	[\xscale]{	\xvoff{\xhoff $16$}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.01$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.02$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.03$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.04$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.05$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.06$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.07$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.08$}}
%
\psfrag{yr1}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $1$}}
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $2$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $3$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $4$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $5$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $6$}}
\psfrag{yr7}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $7$}}
\psfrag{yr8}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $8$}}

==> figures/US-new-positives-shade.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{10mm}{\hspace{0mm}{\# Individuals (in thousands)}}}
%
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Daily new positive cases}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{$p_{n}$ -- Smoothing of the above}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Mar}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $10$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $20$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $30$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $40$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $50$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $60$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $70$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $80$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff $90$}}
\psfrag{y11}[r][r]	[\yscale]{	\yvoff{\yhoff $100$}}

==> figures/US-ratio.tex <==
\newcommand{\commonScale}{.75}
%
\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{15mm}{\hspace{0mm}{Growth Rate}}}
%
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{$x_{n}$ -- Growth rate}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Smoothing of the above}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff Mar}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0.95$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $1.00$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $1.05$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $1.10$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $1.15$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $1.20$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $1.25$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $1.30$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $1.35$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff $1.40$}}
\psfrag{y11}[r][r]	[\yscale]{	\yvoff{\yhoff $1.45$}}

==> figures/US-test-all-waves-non-uniform.tex <==
\newcommand{\commonScale}{1}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Stopping Day}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{12mm}{\hspace{0mm}{Delay [days]}}}
%
\psfrag{wav1}[c][c]	[\commonScale]{	\raisebox{0mm}{\hspace{0mm}{\textsc{Second Wave}}}}
\psfrag{wav2}[c][c]	[\commonScale]{	\raisebox{0mm}{\hspace{0mm}{\textsc{Third Wave}}}}
%
\newcommand{\xscale}{.85}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}

%
%
\newcommand{\yscale}{.85}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $\leqslant 10^{-9}$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-8}$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-7}$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-6}$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-5}$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-4}$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-3}$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-2}$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-1}$}}
%
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $10$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $20$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $30$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $40$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $50$}}
\psfrag{yr7}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $60$}}
\psfrag{yr8}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $70$}}
\psfrag{yr9}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $80$}}
\psfrag{yr10}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $90$}}
\psfrag{yr11}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $100$}}
\psfrag{yr12}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $110$}}
\psfrag{yr13}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $120$}}
\psfrag{yr14}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $130$}}
\psfrag{yr15}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $140$}}
\psfrag{yr16}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $150$}}
\psfrag{yr17}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $160$}}
\psfrag{yr18}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $170$}}
\psfrag{yr19}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $180$}}
\psfrag{yr20}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $190$}}
\psfrag{yr21}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $200$}}
\psfrag{yr22}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $210$}}
\psfrag{yr23}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $220$}}
\psfrag{yr24}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $230$}}
\psfrag{yr25}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $240$}}
\psfrag{yr26}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $250$}}
\psfrag{yr27}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $260$}}

==> figures/United_Kingdom-delay-and-fa-vs-thr.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Threshold}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{8mm}{\hspace{0mm}{Delay [days]}}}
%
%
\psfrag{leg1}[l][l]	[\commonScale]{	\raisebox{0mm}{\hspace{-1mm}{Operational Curve}}}
\psfrag{leg2}[l][l]	[\commonScale]{	\raisebox{0mm}{\hspace{-1mm}{$p_{n}$ -- Moving average applied to $\tilde{p}_{n}$}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-5mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff $0$}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff $5$}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff $10$}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff $15$}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff $20$}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff $25$}}
\psfrag{x7}[c][c]	[\xscale]{	\xvoff{\xhoff $30$}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.01$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.02$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.03$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.04$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.05$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $.06$}}
%
\psfrag{yr1}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $0$}}
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $5$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $10$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $15$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $20$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $25$}}

==> figures/United_Kingdom-new-positives-shade.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{10mm}{\hspace{0mm}{\# Individuals (in thousands)}}}
%
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Daily new positive cases}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{$p_{n}$ -- Smoothing of the above}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Mar}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $5$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $10$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $15$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $20$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $25$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $30$}}

==> figures/United_Kingdom-ratio.tex <==
\newcommand{\commonScale}{.75}
%
\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{15mm}{\hspace{0mm}{Growth Rate}}}
%
%
\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{$x_{n}$ -- Growth rate}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-1mm}{Smoothing of the above}}}
%
%
\newcommand{\xscale}{.65}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff Mar}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Apr}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.65}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0.90$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $0.95$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $1.00$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $1.05$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $1.10$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $1.15$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $1.20$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $1.25$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $1.30$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff $1.35$}}
\psfrag{y11}[r][r]	[\yscale]{	\yvoff{\yhoff $1.40$}}

==> figures/United_Kingdom-test-wave-2-non-uniform.tex <==
\newcommand{\commonScale}{1}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Stopping Day}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{12mm}{\hspace{0mm}{Delay [days]}}}
%
\newcommand{\xscale}{.85}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff Oct}}
%
%
\newcommand{\yscale}{.85}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $\leqslant 10^{-9}$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-8}$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-7}$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-6}$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-5}$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-4}$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-3}$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-2}$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10^{-1}$}}
%
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $10$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $20$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $30$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $40$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $50$}}
\psfrag{yr7}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $60$}}
\psfrag{yr8}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $70$}}
\psfrag{yr9}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $80$}}
\psfrag{yr10}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $90$}}
\psfrag{yr11}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $100$}}
\psfrag{yr12}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $110$}}
\psfrag{yr13}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $120$}}
\psfrag{yr14}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $130$}}
\psfrag{yr15}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $140$}}
\psfrag{yr16}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $150$}}
\psfrag{yr17}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $160$}}
\psfrag{yr18}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $170$}}
\psfrag{yr19}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $180$}}
\psfrag{yr20}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $190$}}
\psfrag{yr21}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $200$}}
\psfrag{yr22}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $210$}}
\psfrag{yr23}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $220$}}
\psfrag{yr24}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $230$}}
\psfrag{yr25}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $240$}}
\psfrag{yr26}[l][l]	[\yscale]{	\yvoff{\hspace{-1.5mm} \color[rgb]{0.85,0.33,0.10} $250$}}

==> figures/all-delay-vs-fa.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[1]{	\raisebox{-10mm}{\hspace{0mm}{Delay [days]}}}
\psfrag{yla}[c][c]	[1]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
%
%
\psfrag{leg1}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Albania ($0.52$)}}}
\psfrag{leg2}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Austria ($1.10$)}}}
\psfrag{leg3}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Belgium ($1.52$)}}}
\psfrag{leg4}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Canada ($0.61$)}}}
\psfrag{leg5}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{France ($0.38$)}}}
\psfrag{leg6}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Germany ($0.75$)}}}
\psfrag{leg7}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Hungary ($1.08$)}}}
\psfrag{leg8}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Italy ($2.74$)}}}
\psfrag{leg9}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Netherlands ($2.83$)}}}
\psfrag{leg10}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Norway ($0.51$)}}}
\psfrag{leg11}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Portugal ($0.83$)}}}
\psfrag{leg12}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Spain ($0.35$)}}}
\psfrag{leg13}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{United States ($2.85$)}}}
\psfrag{leg14}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{United Kingdom ($1.55$)}}}
%
%
\psfrag{d1}[c][c]	[.85]{	\raisebox{2mm}{\hspace{-1mm}$\omega = 0.32$}}
\psfrag{d2}[c][c]	[.85]{	\raisebox{2mm}{\hspace{-1mm}$\omega = 11.52$}}
%
%
\newcommand{\xscale}{.85}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-5mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff $0$}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff $10$}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff $20$}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff $30$}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff $40$}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff $50$}}
%
%
\newcommand{\yscale}{.85}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-9}$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-8}$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-7}$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-6}$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-5}$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-4}$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-3}$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-2}$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-1}$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff $1$}}


==> figures/exponential-growth-real-all-legend.tex <==
\newcommand{\commonScale}{.75}

\psfrag{xla}[c][c]	[1]{	\raisebox{-10mm}{\hspace{0mm}{Day}}}
\psfrag{yla}[c][c]	[1]{	\raisebox{10mm}{\hspace{0mm}{New Positives (Normalized and Shifted)}}}
%
%
\psfrag{leg1}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Albania}}}
\psfrag{leg2}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Austria}}}
\psfrag{leg3}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Belgium}}}
\psfrag{leg4}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Canada}}}
\psfrag{leg5}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{France}}}
\psfrag{leg6}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Germany}}}
\psfrag{leg7}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Hungary}}}
\psfrag{leg8}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Italy}}}
\psfrag{leg9}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Netherlands}}}
\psfrag{leg10}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Norway}}}
\psfrag{leg11}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Portugal}}}
\psfrag{leg12}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Spain}}}
\psfrag{leg13}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{United States}}}
\psfrag{leg14}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{United Kingdom}}}
%
%
\psfrag{a1}[l][l]	[.85]{	\raisebox{2mm}{\hspace{-1mm}$\alpha = .40$}}
\psfrag{a2}[l][l]	[.85]{	\raisebox{2mm}{\hspace{-1mm}$\alpha = .06$}}
\psfrag{a3}[l][l]	[.85]{	\raisebox{2mm}{\hspace{-1mm}$\alpha = .01$}}
%
%
\newcommand{\xscale}{.85}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-5mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff $10$}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff $20$}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff $30$}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff $40$}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff $50$}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff $60$}}
\psfrag{x7}[c][c]	[\xscale]{	\xvoff{\xhoff $70$}}
\psfrag{x8}[c][c]	[\xscale]{	\xvoff{\xhoff $80$}}
\psfrag{x9}[c][c]	[\xscale]{	\xvoff{\xhoff $90$}}
\psfrag{x10}[c][c]	[\xscale]{	\xvoff{\xhoff $100$}}
%
%
\newcommand{\yscale}{.85}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $1$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{1}$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{2}$}}

==> figures/growth-rate-sim.tex <==
\newcommand{\commonScale}{1}
%
\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Day}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{13mm}{\hspace{0mm}{Growth Rate}}}
%
%
\psfrag{leg1}[l][l]	[.75]{	\raisebox{0mm}{\hspace{0mm}{Mean sequence $\mu_{1,n}$}}}
\psfrag{leg2}[l][l]	[.75]{	\raisebox{0mm}{\hspace{0mm}{Synthetic growth rate under ${\cal H}_{1}$}}}
\psfrag{leg3}[l][l]	[.75]{	\raisebox{0mm}{\hspace{0mm}{Mean sequence $\mu_{0,n}$}}}
\psfrag{leg4}[l][l]	[.75]{	\raisebox{0mm}{\hspace{0mm}{Synthetic growth rate under ${\cal H}_{0}$}}}
%
%
\newcommand{\xscale}{.80}
\newcommand{\xhoff}{\hspace{-.75mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff $0$}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff $50$}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff $100$}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff $150$}}
%
%
\newcommand{\yscale}{.80}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0.8$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $0.9$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $1.0$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $1.1$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $1.2$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $1.3$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $1.4$}}

==> figures/mean-correlation.tex <==
\newcommand{\commonScale}{1}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Lag [Days]}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{13mm}{\hspace{0mm}{Normalized Correlation}}}
%
\newcommand{\xscale}{.80}
\newcommand{\xhoff}{\hspace{-.75mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff $-100$}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff $-80$}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff $-60$}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff $-40$}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff $-20$}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff $0$}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff $20$}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff $40$}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff $60$}}
\psfrag{x10}[ct][ct]	[\xscale]{	\xvoff{\xhoff $80$}}
\psfrag{x11}[ct][ct]	[\xscale]{	\xvoff{\xhoff $100$}}
%
%
\newcommand{\yscale}{.80}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $-0.50$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $-0.25$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $0$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $0.25$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $0.50$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $0.75$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $1$}}


==> figures/perf-simulation.tex <==
\newcommand{\commonScale}{.85}

\psfrag{xla}[c][c]	[1]{	\raisebox{-10mm}{\hspace{0mm}{Delay [days]}}}
\psfrag{yla}[c][c]	[1]{	\raisebox{14mm}{\hspace{0mm}{Risk}}}
%
%
\psfrag{leg1}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Uncorr. $\sigma = .065$}}}
\psfrag{leg2}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Uncorr. $\sigma = .065$}}}
\psfrag{leg3}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Corr. $\sigma = .065$}}}
\psfrag{leg4}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Corr. $\sigma = .065$}}}
\psfrag{leg5}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Uncorr. $\sigma = .050$}}}
\psfrag{leg6}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Uncorr. $\sigma = .050$}}}
\psfrag{leg7}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Corr. $\sigma = .050$}}}
\psfrag{leg8}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Corr. $\sigma = .050$}}}
\psfrag{leg9}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Uncorr. $\sigma = .035$}}}
\psfrag{leg10}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Uncorr. $\sigma = .035$}}}
\psfrag{leg11}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Corr. $\sigma = .035$}}}
\psfrag{leg12}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Corr. $\sigma = .035$}}}
%
%
\psfrag{d1}[c][c]	[.85]{	\raisebox{2mm}{\hspace{-1mm}$\omega = 0.32$}}
\psfrag{d2}[c][c]	[.85]{	\raisebox{2mm}{\hspace{-1mm}$\omega = 11.52$}}
%
%
\newcommand{\xscale}{.85}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-5mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff $0$}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff $10$}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff $20$}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff $30$}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff $40$}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff $50$}}
\psfrag{x7}[c][c]	[\xscale]{	\xvoff{\xhoff $60$}}
%
%
\newcommand{\yscale}{.85}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-9}$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-8}$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-7}$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-6}$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-5}$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-4}$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-3}$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-2}$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-1}$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff $1$}}


==> figures/replicate-means-Italy-legend.tex <==
\newcommand{\commonScale}{1}
%
\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-10mm}{\hspace{0mm}{Day}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{15mm}{\hspace{0mm}{Growth Rate}}}
%
%
\psfrag{leg1}[l][l]	[.80]{	\raisebox{0mm}{\hspace{1mm}{Growth rate $x_{n}$}}}
\psfrag{leg2}[l][l]	[.80]{	\raisebox{0mm}{\hspace{1mm}{Estimated mean sequence $\{ \widehat{\mu}_{n} \}$}}}
\psfrag{leg3}[l][l]	[.80]{	\raisebox{0mm}{\hspace{1mm}{Critical regime}}}
\psfrag{leg4}[l][l]	[.80]{	\raisebox{0mm}{\hspace{1mm}{Replicas of $\{ \widehat{\mu}_{1,n} \}$}}}
\psfrag{leg5}[l][l]	[.80]{	\raisebox{0mm}{\hspace{1mm}{Synthetic growth rate under ${\cal H}_{1}$}}}
\psfrag{leg6}[l][l]	[.80]{	\raisebox{0mm}{\hspace{1mm}{Single replica of critical regime}}}
\psfrag{leg7}[l][l]	[.80]{	\raisebox{0mm}{\hspace{1mm}{Controlled regime}}}
\psfrag{leg8}[l][l]	[.80]{	\raisebox{0mm}{\hspace{1mm}{Replicas of $\{ \widehat{\mu}_{0,n} \}$}}}
\psfrag{leg9}[l][l]	[.80]{	\raisebox{0mm}{\hspace{1mm}{Synthetic growth rate under ${\cal H}_{0}$}}}
\psfrag{leg10}[l][l]	[.80]{	\raisebox{0mm}{\hspace{1mm}{Single replica of controlled regime}}}
%
%
\newcommand{\xscale}{.80}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{0mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff $50$}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff $100$}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff $150$}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff $200$}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff $250$}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff $300$}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff $350$}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff $400$}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff $450$}}
\psfrag{x10}[ct][ct]	[\xscale]{	\xvoff{\xhoff $500$}}
\psfrag{x11}[ct][ct]	[\xscale]{	\xvoff{\xhoff $550$}}
%
%
\newcommand{\yscale}{.80}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0.90$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $0.95$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $1.00$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $1.05$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $1.10$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $1.15$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $1.20$}}

==> figures/results-letter-v3.tex <==
\newcommand{\commonScale}{.60}

\psfrag{xla}[c][c]	[.75]{	\raisebox{-10mm}{\hspace{0mm}{$\Delta$ [days]}}}
\psfrag{yla}[c][c]	[.75]{	\raisebox{14mm}{\hspace{0mm}{$R$}}}
%
%
\psfrag{leg1}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Scen. 0, $\alpha/\sigma = 0.5$}}}
\psfrag{leg2}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Scen. 0, $\alpha/\sigma = 0.5$}}}
\psfrag{leg3}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Scen. 1, $\alpha/\sigma = 0.5$}}}
\psfrag{leg4}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Scen. 1, $\alpha/\sigma = 0.5$}}}
\psfrag{leg5}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Scen. 1, $\alpha/\sigma = 1$}}}
\psfrag{leg6}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Scen. 1, $\alpha/\sigma = 1$}}}
\psfrag{leg7}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Scen. 2, $\alpha/\sigma = 0.5$}}}
\psfrag{leg8}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Scen. 2, $\alpha/\sigma = 0.5$}}}
\psfrag{leg9}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Scen. 2, $\alpha/\sigma = 1$}}}
\psfrag{leg10}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Scen. 2, $\alpha/\sigma = 1$}}}
%
%
\newcommand{\xscale}{.75}
\newcommand{\xhoff}{\hspace{-1mm}}
\newcommand{\xvoff}{\raisebox{-6mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff $0$}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff $5$}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff $10$}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff $15$}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff $20$}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff $25$}}
\psfrag{x7}[c][c]	[\xscale]{	\xvoff{\xhoff $30$}}
%
%
\newcommand{\yscale}{.75}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-9}$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-8}$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-7}$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-6}$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-5}$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-4}$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-3}$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-2}$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-1}$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff $1$}}

==> figures/us-states-MAST.tex <==
\newcommand{\commonScale}{.60}

\psfrag{xla}[c][c]	[.75]{	\raisebox{-12mm}{\hspace{0mm}{Stopping Day}}}
\psfrag{yla}[c][c]	[.75]{	\raisebox{14mm}{\hspace{0mm}{MAST}}}
%
%
\psfrag{leg1}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{California}}}
\psfrag{leg2}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Florida}}}
\psfrag{leg3}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Illinois}}}
\psfrag{leg4}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Ohio}}}
\psfrag{leg5}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{North Carolina}}}
\psfrag{leg6}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Michigan}}}
\psfrag{leg7}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Arizona}}}
\psfrag{leg8}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Massachusetts}}}
\psfrag{leg9}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Indiana}}}
\psfrag{leg10}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Tennessee}}}
%
%
\newcommand{\xscale}{.75}
\newcommand{\xhoff}{\hspace{-1mm}}
\newcommand{\xvoff}{\raisebox{-6mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff Oct}}
\psfrag{x7}[c][c]	[\xscale]{	\xvoff{\xhoff Nov}}
\psfrag{x8}[c][c]	[\xscale]{	\xvoff{\xhoff Dec}}
\psfrag{year}[c][c]	[\xscale]{	\raisebox{-10mm}{\xhoff 2020}}
%
%
\newcommand{\yscale}{.75}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $50$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $100$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $150$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $200$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $250$}}
%
%
\psfrag{min}[lc][lb]	[.50]{	\raisebox{8mm}{\hspace{-4mm}{Smallest Thr.}}}
\psfrag{max}[lc][lb]	[.50]{	\raisebox{2mm}{\hspace{-4mm}{Largest Thr.}}}
